Measurements of the Rate of Type Ia Supernovae at Redshift z < ~0.3 from the SDSS-II Supernova Survey

We present a measurement of the volumetric Type Ia supernova (SN Ia) rate based on data from the Sloan Digital Sky Survey II (SDSS-II) Supernova Survey. The adopted sample of supernovae (SNe) includes 516 SNe Ia at redshift z \lesssim 0.3, of which 270 (52%) are spectroscopically identified as SNe Ia. The remaining 246 SNe Ia were identified through their light curves; 113 of these objects have spectroscopic redshifts from spectra of their host galaxy, and 133 have photometric redshifts estimated from the SN light curves. Based on consideration of 87 spectroscopically confirmed non-Ia SNe discovered by the SDSS-II SN Survey, we estimate that 2.04+1.61-0.95 % of the photometric SNe Ia may be misidentified. The sample of SNe Ia used in this measurement represents an order of magnitude increase in the statistics for SN Ia rate measurements in the redshift range covered by the SDSS-II Supernova Survey. If we assume a SN Ia rate that is constant at low redshift (z < 0.15), then the SN observations can be used to infer a value of the SN rate of rV = (2.69+0.34+0.21-0.30-0.01) x10^{-5} SNe yr^{-1} Mpc-3 (H0 /(70 km s^{-1} Mpc^{-1}))^{3} at a mean redshift of ~ 0.12, based on 79 SNe Ia of which 72 are spectroscopically confirmed. However, the large sample of SNe Ia included in this study allows us to place constraints on the redshift dependence of the SN Ia rate based on the SDSS-II Supernova Survey data alone. Fitting a power-law model of the SN rate evolution, r_V(z) = A_p x ((1 + z)/(1 + z0))^{\nu}, over the redshift range 0.0 < z < 0.3 with z0 = 0.21, results in A_p = (3.43+0.15-0.15) x 10^{-5} SNe yr^{-1} Mpc-3 (H0 /(70 km s^{-1} Mpc^{-1}))^{3} and \nu = 2.04+0.90-0.89.

==> tab2.tex <==
\begin{deluxetable}{rcrrcc}
\tablecolumns{6}
\tabletypesize{\small}
\singlespace
\tablewidth{0pc} 
\tablecaption{Confirmed SNe Ia in the Rate Sample
\label{tab:snerates2_conf}
}
\tablehead{
\colhead{SN ID} & 
\colhead{IAU Name} &    
\colhead{$\alpha_{\mathrm{J2000}}$} &    
\colhead{$\delta_{\mathrm{J2000}}$} & 
\colhead{Redshift} &
\colhead{Fitprob} \\ 

\colhead{} & 
\colhead{} & 
\colhead{[degrees]} &    
\colhead{[degrees]} & 
\colhead{} &
\colhead{}

}
\renewcommand{\arraystretch}{1.5}
\startdata
%\input{tabrates2_sne_confirmed.dat}
762 & 2005eg & 15.53518 & -0.87907 & 0.191 & 0.945 \\
1032 & 2005ez & 46.79565 & +1.11952 & 0.130 & 0.541 \\
1112 & 2005fg & 339.01761 & -0.37527 & 0.258 & 0.792 \\
1166 & \nodata & 9.35560 & +0.97320 & 0.382 & 0.992 \\
1241 & 2005ff & 337.67249 & -0.77664 & 0.090 & 0.988 \\
1253 & 2005fd & 323.79895 & +0.16305 & 0.262 & 0.834 \\
1371 & 2005fh & 349.37375 & +0.42929 & 0.119 & 0.995 \\
1580 & 2005fb & 45.32296 & -0.64412 & 0.183 & 1.000 \\
1688 & \nodata & 321.35767 & +0.32447 & 0.359 & 0.183 \\
2017 & 2005fo & 328.94327 & +0.59343 & 0.262 & 0.972 \\
2031 & 2005fm & 312.04312 & -1.17149 & 0.153 & 0.894 \\
2165 & 2005fr & 17.09165 & -0.09639 & 0.288 & 0.930 \\
2246 & 2005fy & 50.09031 & -0.88564 & 0.195 & 0.904 \\
2308 & 2005ey & 34.27273 & +0.28020 & 0.148 & 0.960 \\

\enddata
\tablecomments{See electronic version for full table.}
\end{deluxetable}



==> tab3.tex <==
\begin{deluxetable}{rrrcc}
\tablecolumns{5}
\tabletypesize{\small}
\singlespace
\tablewidth{0pc} 
\tablecaption{SNe with Spectroscopic Redshifts in the Rate Sample
\label{tab:snerates2_105}
}
\tablehead{
\colhead{SN ID} & 
\colhead{$\alpha_{\mathrm{J2000}}$} &    
\colhead{$\delta_{\mathrm{J2000}}$} & 
\colhead{Redshift} &
\colhead{Fitprob} \\ 

\colhead{} & 
\colhead{[degrees]} &    
\colhead{[degrees]} & 
\colhead{} &
\colhead{}

}
\renewcommand{\arraystretch}{1.5}
\startdata
%\input{tabrates2_sne_105.dat}
703 & 336.21786 & +0.65059 & 0.300 & 0.976 \\
779 & 26.67369 & -1.02072 & 0.238 & 0.986 \\
911 & 38.69067 & -0.11571 & 0.208 & 0.930 \\
1008 & 28.27810 & +1.11369 & 0.226 & 0.974 \\
1415 & 6.10647 & +0.59921 & 0.212 & 0.924 \\
1740 & 5.40428 & -0.88099 & 0.167 & 0.013 \\
2057 & 320.39969 & -0.31708 & 0.212 & 0.512 \\
2081 & 337.30505 & -1.20783 & 0.252 & 0.753 \\
2162 & 15.44242 & -0.13368 & 0.173 & 0.777 \\
2532 & 27.74742 & -0.23427 & 0.270 & 0.913 \\
2632 & 45.59013 & -1.22610 & 0.296 & 0.044 \\
2639 & 330.46411 & +0.66447 & 0.215 & 0.278 \\
2734 & 48.20686 & -0.69485 & 0.303 & 0.149 \\
2806 & 45.26690 & +0.27364 & 0.301 & 0.340 \\

\enddata
\tablecomments{See electronic version for full table.}
\end{deluxetable}




==> tab4.tex <==
\begin{deluxetable}{rrrccc}
\tablecolumns{6}
\tabletypesize{\small}
\singlespace
\tablewidth{0pc} 
\tablecaption{SNe with Photometric Redshifts in the Rate Sample
\label{tab:snerates2_photoz}
}
\tablehead{
\colhead{SN ID} & 
\colhead{$\alpha_{\mathrm{J2000}}$} &    
\colhead{$\delta_{\mathrm{J2000}}$} & 
\colhead{Redshift} &
\colhead{Redshift Error} &
\colhead{Fitprob} \\ 

\colhead{} & 
\colhead{[degrees]} &    
\colhead{[degrees]} & 
\colhead{} &
\colhead{}
}
\renewcommand{\arraystretch}{1.5}
\startdata
%\input{tabrates2_sne_photoz.dat}
822 & 40.56070 & -0.86217 & 0.220 & 0.018 & 0.090 \\
1342 & 346.52740 & +0.11688 & 0.283 & 0.026 & 0.962 \\
1403 & 359.70386 & +0.43188 & 0.341 & 0.034 & 0.112 \\
1658 & 357.50443 & +0.65006 & 0.256 & 0.025 & 0.836 \\
1899 & 323.34305 & -0.70642 & 0.341 & 0.037 & 0.005 \\
2784 & 28.07526 & -0.04169 & 0.381 & 0.021 & 0.488 \\
2855 & 16.17518 & -0.35642 & 0.233 & 0.016 & 0.978 \\
3206 & 13.57741 & +0.41816 & 0.387 & 0.031 & 0.003 \\
3368 & 44.45594 & +1.23082 & 0.320 & 0.035 & 0.831 \\
3417 & 314.27606 & +0.97825 & 0.262 & 0.016 & 0.413 \\
3506 & 336.25064 & -0.97821 & 0.211 & 0.011 & 0.963 \\
3945 & 346.00906 & -0.28307 & 0.260 & 0.017 & 0.070 \\
3975 & 29.82097 & +0.20364 & 0.399 & 0.019 & 0.002 \\
3983 & 7.27582 & -0.25663 & 0.279 & 0.021 & 0.220 \\


\enddata
\tablecomments{See electronic version for full table.}
\end{deluxetable}



